Depth Pro: Sharp Monocular Metric Depth in Less Than a Second

We present a foundation model for zero-shot metric monocular depth estimation. Our model, Depth Pro, synthesizes high-resolution depth maps with unparalleled sharpness and high-frequency details. The predictions are metric, with absolute scale, without relying on the availability of metadata such as camera intrinsics. And the model is fast, producing a 2.25-megapixel depth map in 0.3 seconds on a standard GPU. These characteristics are enabled by a number of technical contributions, including an efficient multi-scale vision transformer for dense prediction, a training protocol that combines real and synthetic datasets to achieve high metric accuracy alongside fine boundary tracing, dedicated evaluation metrics for boundary accuracy in estimated depth maps, and state-of-the-art focal length estimation from a single image. Extensive experiments analyze specific design choices and demonstrate that Depth Pro outperforms prior work along multiple dimensions. We release code and weights at https://github.com/apple/ml-depth-pro

==> fig/3dphoto.tex <==
\begin{figure}[htbp]
  \centering
  \captionsetup[sub]{labelformat=empty}
  \fboxrule=0.7pt\relax
  \fboxsep=0pt\relax
  \subfloat[]{%
    \includegraphics[width=0.24\textwidth]{fig/3dphoto/reference_image.jpg}
  }
  \subfloat[]{%
    \stackinset{r}{1.5pt}{b}{1.5pt}{
      \color{blue_c}\fbox{\includegraphics[width=0.10\textwidth]{fig/3dphoto/depth_pro_crp.jpg}}}{%
      \includegraphics[width=0.24\textwidth]{fig/3dphoto/depth_pro_image.jpg}}%
  }
  \hspace{0.5mm}%
  \subfloat[]{%
    \stackinset{r}{1.5pt}{b}{1.5pt}{
      \color{green_c}\fbox{\includegraphics[width=0.10\textwidth]{fig/3dphoto/marigold_crp.jpg}}}{%
      \includegraphics[width=0.24\textwidth]{fig/3dphoto/marigold_image.jpg}}%
  }
  \hspace{0.5mm}%
  \subfloat[]{%
    \stackinset{r}{1.5pt}{b}{1.5pt}{
      \color{red_c}\fbox{\includegraphics[width=0.10\textwidth]{fig/3dphoto/depth_anything_crp.jpg}}}{%
      \includegraphics[width=0.24\textwidth]{fig/3dphoto/depth_anything_image.jpg}}%
  }

  % Second row
  \vspace{-5.5mm}
  \subfloat[Reference]{%
    \includegraphics[width=0.24\textwidth]{fig/3dphoto/reference_image3.jpg}
  }
  \subfloat[Depth Pro (Ours)]{%
    \stackinset{l}{1.5pt}{t}{1.5pt}{
      \color{blue_c}\fbox{\includegraphics[width=0.10\textwidth]{fig/3dphoto/depth_pro_crp3.jpg}}}{%
      \includegraphics[width=0.24\textwidth]{fig/3dphoto/depth_pro_image3.jpg}}%
  }
  \hspace{0.5mm}%
  \subfloat[Marigold]{%
    \stackinset{l}{1.5pt}{t}{1.5pt}{
      \color{green_c}\fbox{\includegraphics[width=0.10\textwidth]{fig/3dphoto/marigold_crp3.jpg}}}{%
      \includegraphics[width=0.24\textwidth]{fig/3dphoto/marigold_image3.jpg}}%
  }
  \hspace{0.5mm}%
  \subfloat[Depth Anything]{%
    \stackinset{l}{1.5pt}{t}{1.5pt}{
      \color{red_c}\fbox{\includegraphics[width=0.10\textwidth]{fig/3dphoto/depth_anything_crp3.jpg}}}{%
      \includegraphics[width=0.24\textwidth]{fig/3dphoto/depth_anything_image3.jpg}}%
  }
  \vspace{-1mm}
  \caption{\textbf{Comparison on novel view synthesis.} We compare Depth Pro, Marigold~\citep{Ke2024:CVPR}, and Depth Anything~\citep{Yang2024:CVPR} on novel view synthesis by plugging depth predictions into 3D Photo~\citep{Shih2020:CVPR}. Depth Pro's sharper and more accurate depth maps yields novel views with significantly less artifacts. Marigold can produce detailed depth maps at significantly higher cost than our method; furthermore, their borders do not match accurately with the RGB images, resulting in artifacts in several images. Depth Anything also suffers from misalignment between the RGB image and the estimated depth map, as demonstrated in the flying pixels in the second row; it also fails to properly understand the shape of the glass in the first row.}
  \label{fig:applications_3dphoto}
\end{figure}

==> fig/boundary_problems.tex <==
\begin{figure}
\scriptsize
\centering
\begin{subfigure}{0.22\textwidth}
    \includegraphics[width=\linewidth]  {fig/edges/boundary_problems/warping_am2k_image_metric3d_v2g.pdf}
    \caption{Image} \label{fig:boundary_problems:a}
\end{subfigure}%
\hspace*{\fill} 
\begin{subfigure}{0.22\textwidth}
    \includegraphics[width=\linewidth]  {fig/edges/boundary_problems/warping_am2k_pred_metric3d_v2g.pdf}
    \caption{Metric3d-v2 (G)} \label{fig:boundary_problems:b}
\end{subfigure}%
\hspace*{\fill} 
\begin{subfigure}{0.22\textwidth}
    \includegraphics[width=\linewidth]  {fig/edges/boundary_problems/warping_am2k_warping_metric3d_v2g.pdf}
    \caption{Warping} \label{fig:boundary_problems:c}
\end{subfigure}%
\hspace*{\fill} 
\begin{subfigure}{0.22\textwidth}
    \includegraphics[width=\linewidth]  {fig/edges/boundary_problems/warping_am2k_matting_metric3d_v2g.pdf}
    \caption{Alpha Matte} \label{fig:boundary_problems:d}
\end{subfigure}%
\caption{
\textbf{On the importance of accurate depth boundary prediction.}
We show in (b) the depth prediction from Metric3D-v2 (G)~\cite{Hu2024:arxiv} on an image (a) from the AM-2k~\cite{Li2022:IJCV} dataset. The incorrect prediction of depth boundaries severely hinders applications such as image warping as illustrated in (c). We propose to leverage high-quality 2D annotations (d) to quantitatively evaluate this issue.
}
 \label{fig:boundary_problems}
\end{figure}

==> tab/arch_1536.tex <==
\begin{table}[htbp]
  \centering
  \begin{tabular}{@{}lllllll@{}}
    Model & \multicolumn{1}{p{0.5cm}}{Input \newline size} & AbsRel $\downarrow$ & Log10 $\downarrow$ & \multicolumn{1}{p{0.5cm}}{Edge \newline F1$\uparrow$} & \multicolumn{1}{p{0.5cm}}{Edge0 \newline R$\uparrow$} & \multicolumn{1}{p{0.5cm}}{Edge1 \newline R$\uparrow$}\\
    \midrule
    
    Seg-Anything ViT-L & 1536 & 0.122 & 0.375 & 0.044 & 0.083 & \underline{0.005}\\
    ConvNext-xxlarge & 1536 & 0.134 & 0.329 & 0.029 & 0.049 & 0.002\\
    ConvNextV2-huge & 1536 & 0.126 & 0.323 & 0.089 & 0.075 & 0.003\\
    SWINv2-large & 1536 & 0.151 & 0.259 & 0.029 & 0.048 & 0.001\\

    MViTv2-large & 1280 & OOM & OOM & OOM & OOM & OOM\\
    MViTv2-large & 1024 & 0.122 & 0.272 & 0.001 & 0.051 & \bf{0.007}\\

    ViT-B16-mae & 1536 & 0.063 & 0.205 & 0.068 & 0.078 & \underline{0.005}\\
    ViT-L16-mae & 1536 & 0.040 & 0.124 & 0.170 & \underline{0.086} & \underline{0.005}\\
    ViT-L16-beitv2 & 1536 & OOM & OOM & OOM & OOM & OOM\\
    ViT-L16-beitv2 & 1024 & \underline{0.038} & 0.104 & 0.153 & 0.075 & 0.002\\

    \midrule
    SPN-ViT-B-mae & 1536 & 0.061 & 0.185 & 0.143 & 0.077 & 0.004\\  
    SPN-ViT-L-beitv2 & 1536 & 0.040 & 0.117 & 0.222 & 0.071 & 0.002\\
    ViT-L-beitv2 + SPN-ViT-L-beitv2 & 1536 & 0.041 & 0.142 & 0.218 & 0.065 & 0.002\\
    ViT-L-eva + SPN-ViT-L-beitv2  & 1536 & 0.039 & \bf{0.091} & \underline{0.246} & 0.073 & 0.002\\
    ViT-L-eva + SPN-ViT-B-mae & 1536 & 0.040 & \underline{0.095} & 0.223 & \bf{0.088} & \underline{0.005}\\
    ViT-L-eva + SPN-ViT-L-mae & 1536 & \bf{0.037} & 0.115 & \bf{0.256} & 0.081 & 0.004\\
  \bottomrule
  \end{tabular}
  \caption{\textbf{Comparison to other high-resolution architectures.} Comparison of models with 1536$\times$1536 resolution trained for 20 epochs with fixed epoch length 72K samples per epoch on 5 RGB-D datasets: Keystone, HRWSI, RedWeb, TartanAir, Hypersim. OOM - means out of memory on V100-32GB GPU. We tried different pretrained weights for ViT models: EVA-clip~\cite{Sun2023:arxiv}, BeiTv2~\cite{Peng2022:arxiv} and MAE~\cite{He2022:CVPR}.
  }
  \label{tab:arch1536}
\end{table}

==> tab/sota_0shot_metric2.tex <==
\begin{table}[htbp]
    \newcolumntype{Y}{S[table-format=2.1,table-auto-round]}
    \centering
    \scriptsize
    \begin{tabularx}{\linewidth}{X@{\hspace{3mm}}Y*{10}{@{\hspace{2mm}}Y}@{\hspace{2mm}}|Y}
\toprule
Method \textbackslash \ Dataset $\delta_1\uparrow$ 
& {Booster} & {DDAD} & {DIODE-I} & {ETH} & {iBims} & {KITTI} & {Middleb.} & {NuS} & {NYUv2} & {Sintel} & {SunRGB} & {\textbf{Rank}} \\
\midrule
DepthAnything~\cite{Yang2024:arxiv}$^1$ &   \cellfirst{96.9} &               23.4 &               28.9 &                9.6 &               71.4 &  \cellsecond{97.8} &               39.3 &               36.1 &   \cellthird{98.4} &                6.9 &               67.8 &               5.5 \\
Metric3D v2 (L) ~\cite{Hu2024:arxiv}    &                4.0 &                nan &   \cellfirst{97.4} &   \cellthird{82.4} &               86.5 &   \cellthird{97.1} &                7.0 &   \cellthird{65.8} &               95.0 &               19.5 &   \cellfirst{84.4} &               4.8 \\
Metric3D v2 (G) ~\cite{Hu2024:arxiv}    &                1.1 &                nan &  \cellsecond{96.7} &   \cellfirst{88.6} &   \cellthird{90.6} &               95.6 &                1.9 &               63.8 &               95.7 &   \cellfirst{41.4} &  \cellsecond{82.4} &  \cellsecond{4.4} \\
PatchFusion ~\cite{Li2023:arxiv}        &               22.6 &                nan &                nan &               48.4 &               58.3 &                1.5 &               49.9 &                9.3 &               87.3 &               14.0 &               33.9 &               7.7 \\
UniDepth ~\cite{Piccinelli2024:CVPR}    &               29.1 &                nan &   \cellthird{95.5} &               20.0 &               23.6 &   \cellfirst{98.4} &               36.1 &  \cellsecond{69.5} &  \cellsecond{98.4} &               16.4 &               53.0 &               5.4 \\
UniDepth v2 ~\cite{Piccinelli2024:CVPR} &               52.2 &                nan &               93.5 &  \cellsecond{86.0} &  \cellsecond{91.2} &                nan &                nan &   \cellfirst{73.8} &   \cellfirst{98.7} &  \cellsecond{36.5} &               55.9 &   \cellthird{4.5} \\
ZeroDepth ~\cite{Guizilini2023:ICCV}    &                nan &   \cellfirst{77.2} &               32.3 &                nan &               74.6 &               85.1 &               44.4 &               29.8 &               71.3 &               12.9 &                nan &               7.3 \\
ZoeDepth ~\cite{Bhat2023:arxiv}         &               25.5 &                0.1 &               28.2 &               33.1 &               65.8 &                0.0 &   \cellthird{56.0} &                0.1 &               95.5 &                9.5 &               56.9 &               7.0 \\
\midrule
Ours-S3 M 7k69mdqp5m                    &  \cellsecond{62.8} &  \cellsecond{65.5} &               39.3 &               65.6 &               90.0 &               10.3 &  \cellsecond{73.4} &               45.9 &               90.8 &               25.4 &               65.2 &               4.5 \\
Ours-S3 G s5rs4eprix                    &   \cellthird{56.0} &   \cellthird{64.6} &               39.9 &               78.9 &   \cellfirst{92.6} &                1.2 &   \cellfirst{79.8} &               39.6 &               94.3 &   \cellthird{27.4} &   \cellthird{73.2} &   \cellfirst{4.0} \\
\bottomrule
\end{tabularx}
  \caption{\textbf{Comparison on zero-shot metric depth.} (SOTA metric depth estimators on several benchmarks). For fair comparison, all reported results were reproduced in our environment. \footnotesize{$^1$, $^2$ is DepthAnything~\cite{Yang2024:arxiv} model fine-tuned for metric depth on NYU$^1$ and Kitti$^2$, respectively. $^3$ is fine-tuned on both NYU and Kitti. For Metric3D v2, we compare results of ViT-giant2 (G) and ViT-Large (L) models. Detailed metrics are available in the supplementary material.}}
  \label{tab:sota_0shot_metric}
\end{table}

\begin{table}[htbp]
    \newcolumntype{Y}{S[table-format=2.1,table-auto-round]}
    \centering
    \scriptsize
    \begin{tabularx}{\linewidth}{X@{\hspace{3mm}}Y*{10}{@{\hspace{2mm}}Y}@{\hspace{2mm}}|Y}
\toprule
Method \textbackslash \ Dataset $\delta_1\uparrow$ 
& {Booster} & {DDAD} & {DIODE-I} & {ETH} & {iBims} & {KITTI} & {Middleb.} & {NuS} & {NYUv2} & {Sintel} & {SunRGB} & {\textbf{Rank}} \\
\midrule
DepthAnything~\cite{Yang2024:arxiv}$^1$ &   \cellfirst{96.9} &   \cellthird{23.4} &               28.9 &                9.6 &               71.4 &  \cellsecond{97.8} &               39.3 &               36.1 &   \cellthird{98.4} &                6.9 &  \cellsecond{67.8} &               4.3 \\
Metric3D v2 (L) ~\cite{Hu2024:arxiv}    &                4.0 &                nan &   \cellfirst{97.4} &  \cellsecond{82.4} &   \cellthird{86.5} &   \cellthird{97.1} &                7.0 &   \cellthird{65.8} &               95.0 &   \cellthird{19.5} &   \cellfirst{84.4} &   \cellthird{3.9} \\
PatchFusion ~\cite{Li2023:arxiv}        &               22.6 &                nan &                nan &               48.4 &               58.3 &                1.5 &   \cellthird{49.9} &                9.3 &               87.3 &               14.0 &               33.9 &               6.1 \\
UniDepth ~\cite{Piccinelli2024:CVPR}    &               29.1 &                nan &  \cellsecond{95.5} &               20.0 &               23.6 &   \cellfirst{98.4} &               36.1 &  \cellsecond{69.5} &  \cellsecond{98.4} &               16.4 &               53.0 &               4.3 \\
UniDepth v2 ~\cite{Piccinelli2024:CVPR} &   \cellthird{52.2} &                nan &   \cellthird{93.5} &   \cellfirst{86.0} &   \cellfirst{91.2} &                nan &                nan &   \cellfirst{73.8} &   \cellfirst{98.7} &   \cellfirst{36.5} &               55.9 &  \cellsecond{3.4} \\
ZeroDepth ~\cite{Guizilini2023:ICCV}    &                nan &   \cellfirst{77.2} &               32.3 &                nan &               74.6 &               85.1 &               44.4 &               29.8 &               71.3 &               12.9 &                nan &               5.6 \\
ZoeDepth ~\cite{Bhat2023:arxiv}         &               25.5 &                0.1 &               28.2 &               33.1 &               65.8 &                0.0 &  \cellsecond{56.0} &                0.1 &               95.5 &                9.5 &               56.9 &               5.4 \\
\midrule
Ours-S3 M 7k69mdqp5m                    &  \cellsecond{62.8} &  \cellsecond{65.5} &               39.3 &   \cellthird{65.6} &  \cellsecond{90.0} &               10.3 &   \cellfirst{73.4} &               45.9 &               90.8 &  \cellsecond{25.4} &   \cellthird{65.2} &   \cellfirst{3.1} \\
\bottomrule
\bottomrule
\end{tabularx}
  \caption{\textbf{Comparison on zero-shot metric depth.} (SOTA metric depth estimators on several benchmarks). For fair comparison, all reported results were reproduced in our environment. \footnotesize{$^1$, $^2$ is DepthAnything~\cite{Yang2024:arxiv} model fine-tuned for metric depth on NYU$^1$ and Kitti$^2$, respectively. $^3$ is fine-tuned on both NYU and Kitti. For Metric3D v2, we compare results of ViT-giant2 (G) and ViT-Large (L) models. Detailed metrics are available in the supplementary material.}}
  \label{tab:sota_0shot_metric}
\end{table}

==> tab/sota_0shot_relative.tex <==
\begin{table}[htbp]
  \vspace{1.5mm}
  \label{tab:reldepth}
  \centering
  \scriptsize
  \begin{tabular}{@{}lrrrrrrrr@{}}
    Method & \multicolumn{2}{p{1.7cm}}{NYUv2}&\multicolumn{2}{p{1.7cm}}{KITTI}& \multicolumn{2}{p{1.7cm}}{ETH3D}& \multicolumn{2}{p{1.7cm}}{Diode(Indoor)}\\
    & RelAbs$\downarrow$ & $\delta$1$\uparrow$ & RelAbs$\downarrow$ & $\delta$1$\uparrow$ & RelAbs$\downarrow$ & $\delta$1$\uparrow$ & RelAbs$\downarrow$ & $\delta$1$\uparrow$ \\
    \midrule
    DPT~\cite{Ranftl2021:ICCV} & 0.125 & 0.861 & 0.190 & 0.760 & 0.751 & 0.253 & 0.068 & 0.947 \\
    DepthAnything~\cite{Yang2024:arxiv} & \cellsecond{0.043} & \cellsecond{0.980} & 0.080 & 0.942 & 0.671 & 0.246 & 0.111 & 0.896 \\
    Marigold~\cite{Ke2023:arxiv}  & 0.056 & 0.962 & 0.118 & 0.863 & 0.129 & 0.862 & 0.045 & 0.970 \\
    Metric3D~\cite{Yin2023:ICCV} & 0.051 & 0.966 & \cellsecond{0.052} & \cellsecond{0.977} & 0.158 & 0.853 & 0.046 & 0.969 \\
    Metric3D v2~\cite{Hu2024:arxiv} & \cellfirst{0.042} & \cellfirst{0.981} & \cellfirst{0.042} & \cellfirst{0.980} & \cellsecond{0.016} & \cellthird{0.993} & \cellfirst{0.020} & \cellfirst{0.993} \\
    PatchFusion~\cite{Li2023:arxiv} & 0.065 & 0.962 & 0.097 & 0.910 & \cellthird{0.017} & \cellsecond{0.995} & \cellthird{0.041} & 0.972 \\
    ZeroDepth~\cite{Guizilini2023:ICCV} & 0.115 & 0.863 & 0.102 & 0.895 & OOM & OOM & 0.070 & 0.935 \\
    ZoeDepth~\cite{Bhat2023:arxiv} & \cellsecond{0.043} & \cellfirst{0.981} & \cellthird{0.055} & \cellthird{0.975} & 0.085 & 0.934 & 0.045 & \cellthird{0.973} \\
    \midrule
    Depth Pro (Ours) & \cellthird{0.052} & \cellthird{0.975} & 0.066 & 0.956 & \cellfirst{0.009} & \cellfirst{0.999} & \cellsecond{0.036} & \cellsecond{0.980} \\
    \bottomrule
    \\
  \end{tabular}
  \\
  \begin{tabular}{@{}lrrrrrrrr@{}}
    Method & \multicolumn{2}{p{1.7cm}}{InStereo2k}&\multicolumn{2}{p{1.7cm}}{Sintel}&\multicolumn{2}{p{1.7cm}}{Middlebury}&\multicolumn{2}{p{1.7cm}}{Booster}\\
    & RelAbs$\downarrow$ & $\delta$1$\uparrow$ & RelAbs$\downarrow$ & $\delta$1$\uparrow$ &RelAbs$\downarrow$ & $\delta$1$\uparrow$ & RelAbs$\downarrow$ & $\delta$1$\uparrow$ \\
    \midrule
    DPT~\cite{Ranftl2021:ICCV} & 0.049 & 0.984 & 0.784 & 0.520 & 0.090 & 0.912 & 0.089 & 0.941 \\
    DepthAnything~\cite{Yang2024:arxiv} & \cellthird{0.044} & \cellthird{0.987} & \cellsecond{0.429} & 0.597 & 0.093 & 0.943 & 0.104 & 0.913 \\
    Marigold~\cite{Ke2023:arxiv}  & 0.081 & 0.951 & 0.548 & \cellsecond{0.646} & 0.042 & \cellthird{0.991} & \cellsecond{0.042} & \cellthird{0.983} \\
    Metric3D~\cite{Yin2023:ICCV} & 0.051 & 0.982 & 0.733 & 0.530 & 0.132 & 0.889 & 0.087 & 0.921 \\
    Metric3D v2~\cite{Hu2024:arxiv} & \cellfirst{0.027} & \cellfirst{0.995} & \cellfirst{0.316} & \cellfirst{0.798} & \cellfirst{0.027} & \cellfirst{0.997} & \cellfirst{0.026} & \cellfirst{0.993} \\
    PatchFusion~\cite{Li2023:arxiv} & - & - & \cellthird{0.524} &\cellthird{0.643} & 0.059 & 0.978 & \cellthird{0.065} & 0.953 \\
    ZeroDepth~\cite{Guizilini2023:ICCV} & 0.065 & 0.970 & 0.742 & 0.531 & 0.098 & 0.917 & OOM & OOM \\
    ZoeDepth~\cite{Bhat2023:arxiv} & 0.048 & 0.983 & 0.528 & 0.630 & \cellthird{0.051} & 0.985 & \cellthird{0.065} & 0.959 \\
    \midrule
    Depth Pro (Ours) & \cellthird{0.035} & \cellsecond{0.992} & 0.787 & 0.634 & \cellsecond{0.034} & \cellsecond{0.996} & \cellsecond{0.042} & \cellsecond{0.985} \\
    \bottomrule
  \end{tabular}
    \caption{Relative depth (SOTA affine-invariant depth estimators on several zero-shot benchmarks). For fair comparison, all reported results were reproduced in our environment.
  }
\end{table}

==> tab/sota_pc.tex <==
\begin{table}[htbp]
    \caption{Point cloud study}
    \label{tab:point_cloud}
    \centering
\begin{tabular}{llllll}
\multicolumn{3}{c}{DIODE-INDOOR} \\
\toprule
Method &   F$\uparrow$ &       IoU$\uparrow$ \\
\midrule
DA-Indoor~\cite{Yang2024:arxiv}$^1$  &               0.130  &               0.076 \\
DA-Outdoor~\cite{Yang2024:arxiv}$^2$ &                      &                     \\
Metric3D ~\cite{Yin2023:ICCV}        &               0.154  &               0.093 \\
Metric3D v2 (G) ~\cite{Hu2024:arxiv} &   \cellfirst{0.347}  &   \cellfirst{0.239} \\
Metric3D v2 (L) ~\cite{Hu2024:arxiv} &   \cellsecond{0.327} &  \cellsecond{0.225} \\
PatchFusion ~\cite{Li2023:arxiv}     &                      &                     \\
ZeroDepth ~\cite{Guizilini2023:ICCV} &                0.109 &               0.063 \\
ZoeDepth ~\cite{Bhat2023:arxiv}      &                0.144 &               0.085 \\
\hline
Ours-S3, 7k69mdqp5m                  &    \cellthird{0.170} &   \cellthird{0.106} \\
\\
\multicolumn{3}{c}{Middlebury} \\
    \toprule
     Method &   F$\uparrow$ &       IoU$\uparrow$ \\
    \midrule
DA-Indoor~\cite{Yang2024:arxiv}$^1$  &               0.103 &               0.055 \\
DA-Outdoor~\cite{Yang2024:arxiv}$^2$ &                     &                     \\
Metric3D ~\cite{Yin2023:ICCV}        &               0.067 &               0.036 \\
Metric3D v2 (G) ~\cite{Hu2024:arxiv} &   \cellfirst{0.182} &  \cellsecond{0.101} \\
Metric3D v2 (L) ~\cite{Hu2024:arxiv} &               0.170 &               0.094 \\
PatchFusion ~\cite{Li2023:arxiv}     &               0.084 &               0.044 \\
ZeroDepth ~\cite{Guizilini2023:ICCV} &               0.049 &               0.025 \\
ZoeDepth ~\cite{Bhat2023:arxiv}      &               0.112 &               0.060 \\
\hline
Ours-S3, 7k69mdqp5m                  &               0.090 &               0.048 \\
\\
\multicolumn{3}{c}{ETH3D} \\
\toprule
Method &    F$\uparrow$ &       IoU$\uparrow$ \\
\midrule
DA-Indoor~\cite{Yang2024:arxiv}$^1$  &                     &                     \\
DA-Outdoor~\cite{Yang2024:arxiv}$^2$ &                     &                     \\
Metric3D ~\cite{Yin2023:ICCV}        &              0.303  &               0.219 \\
Metric3D v2 (G) ~\cite{Hu2024:arxiv} &  \cellthird{0.466}  &               0.358 \\
Metric3D v2 (L) ~\cite{Hu2024:arxiv} &  \cellsecond{0.484} &  \cellsecond{0.376} \\
PatchFusion ~\cite{Li2023:arxiv}     &               0.215 &               0.139 \\
ZeroDepth ~\cite{Guizilini2023:ICCV} &                     &                     \\
ZoeDepth ~\cite{Bhat2023:arxiv}      &               0.127 &               0.082 \\
\hline
Ours-S3, 7k69mdqp5m                  &                0.460 &   \cellthird{0.361} \\
\\
\multicolumn{3}{c}{Sun-RGBD} \\
\toprule
Method &    F$\uparrow$ &       IoU$\uparrow$ \\
\midrule
DA-Indoor~\cite{Yang2024:arxiv}$^1$  &               0.200 &               0.115 \\
DA-Outdoor~\cite{Yang2024:arxiv}$^2$ &                     &                     \\
Metric3D ~\cite{Yin2023:ICCV}        &               0.093 &               0.050 \\
Metric3D v2 (G) ~\cite{Hu2024:arxiv} &  \cellsecond{0.244} &  \cellsecond{0.145} \\
Metric3D v2 (L) ~\cite{Hu2024:arxiv} &   \cellthird{0.230} &   \cellthird{0.136} \\
PatchFusion ~\cite{Li2023:arxiv}     &                     &                     \\
ZeroDepth ~\cite{Guizilini2023:ICCV} &                     &                     \\
ZoeDepth ~\cite{Bhat2023:arxiv}      &               0.180 &               0.103 \\
\hline
Ours-S3, 7k69mdqp5m                  &               0.198 &               0.115 \\
\bottomrule
\end{tabular}

\end{table}


==> tab/sota_systems.tex <==
\begin{table}[htbp]

  \label{tab:nyuv2}
  \centering
  \begin{tabular}{@{}lllllllllllll@{}}
    \footnotesize &\multicolumn{2}{c}{DIODE in}&\multicolumn{2}{c}{DIODE out}& \multicolumn{2}{c}{ETH}& \multicolumn{2}{c}{iBims-1}&\multicolumn{2}{c}{Sintel}&\multicolumn{2}{c}{SUNRGB-D}\\
    & REL$\downarrow$ & $\delta$1$\uparrow$ & REL$\downarrow$ & $\delta$1$\uparrow$ & REL$\downarrow$ & $\delta$1$\uparrow$ & REL$\downarrow$ & $\delta$1$\uparrow$ & REL$\downarrow$ & $\delta$1$\uparrow$ & REL$\downarrow$ & $\delta$1$\uparrow$ \\
    \midrule
    DMD~\cite{Saxena2023:arxiv} & \\
    DAnything~\cite{Yang2024:arxiv}$^2$ & \\ 
    Metric3D~\cite{Yin2023:ICCV} & \\ 
    ZoeDepth$^1$~\cite{Bhat2023:arxiv}* & \\ 
    \midrule
    SPN (ours)  & & & & & & & & & & & & \\
  \bottomrule
  \end{tabular}
      \caption{Comparison to state of the art on system level.\\
\footnotesize {$^1$ use proprietary datasets. $^2$ use unlabeled datasets.}
  }
\end{table}

